A QoS Aware Approach to Service-Oriented Communication in Future Automotive Networks

Service-Oriented Architecture (SOA) is about to enter automotive networks based on the SOME/IP middleware and an Ethernet high-bandwidth communication layer. It promises to meet the growing demands on connectivity and flexibility for software components in modern cars. Largely heterogeneous service requirements and time-sensitive network functions make Quality-of-Service (QoS) agreements a vital building block within future automobiles. Existing middleware solutions, however, do not allow for a dynamic selection of QoS. This paper presents a service-oriented middleware for QoS aware communication in future cars. We contribute a protocol for dynamic QoS negotiation along with a multi-protocol stack, which supports the different communication classes as derived from a thorough requirements analysis. We validate the feasibility of our approach in a case study and evaluate its performance in a simulation model of a realistic in-car network. Our findings indicate that QoS aware communication can indeed meet the requirements, while the impact of the service negotiations and setup times of the network remain acceptable provided the cross-traffic during negotiations stays below 70% of the available bandwidth.

==> tex/plots.tex <==
%!TEX root = ../main.tex

\begin{table}
	\centering
	\caption{Single publish-subscribe setup times for the different Service Classes}
	\begin{tabular}{|lll|}
	\hline
	    		& QoS Duration & Last remote added at \\
	IPS(UDP) 	& 75,824us     & 56,92us              \\
	IPS(TCP) 	& 75,824us     & 129,128us            \\
	RTS(AVB) 	& 76,496us     & 94,324us             \\
	\hline
	\end{tabular}
\end{table}


\begin{table}
	\centering
	\caption{Min Max AVG latency in mixed critical network with CT }
	\begin{tabular}{|llll|}
	\hline
	    & Min  & Max   & Avg/Mean \\
	AVB & 34us & 157us & 90us     \\
	TCP & 50us & 790us & 140us    \\
	UDP & 58us & 798us & 156us    \\
	\hline
	\end{tabular}
\end{table}


\begin{figure}
	\centering
		\begin{tikzpicture} 

			\begin{axis}[change y base, y SI prefix=milli, y unit=\milli\second, x unit=\second,xlabel={Simulation time}, ylabel={$L_{End2End}$},  xmin=0.5, xmax=0.8,legend style={font=\scriptsize,at={(.05,.95)},anchor=north west}] 

				%bars for phases
				\draw[green] (0,0.00025) -- ( 2.5, 0.00025);

				\addplot [corered] table {\alltypeslatencyavb} ;%|- (axis cs:0,0) -- cycle; 
				\addplot [coreblue] table {\alltypeslatencytcp};% |- (axis cs:0,0) -- cycle; 
				%\addplot [coregreen] table {\alltypeslatencyudp};% |- (axis cs:0,0) -- cycle; 

				\node[pin=45:{\footnotesize{$L_{AVB_{MAX}}$}}]at (0.5, 0.00025) { };
				\legend{\ac{RTS},\ac{IPS}}%,$IPS(UDP)$}
			\end{axis} 
		\end{tikzpicture}
	\caption{End-to-end latency analysis with different service classes under varying \acl{CT}.}
	\label{fig:latency}
	%\vspace{-7mm}
\end{figure}	


\begin{figure}
	\centering
		\begin{tikzpicture}[extended line/.style={shorten >=-#1,shorten <=-#1}, extended line/.default=1cm] 

			\begin{axis}[change y base, y SI prefix=micro, y unit=\micro\second,xlabel={Subscriber Count}, ylabel={Setup Time}, xmin=1, xmax=10, legend style={font=\scriptsize,at={(.05,.95)},anchor=north west}] 

				\draw [extended line=5cm] (5,0.000100536) -- (4,0.000100536);
				\addplot [mark=o,corered] table {\pubsubcountone} ;
				\addplot [mark=o,coreblue] table {\pubsubcounttwo} ;
				\addplot [mark=o,coregreen] table {\pubsubcountthree} ;
				\addplot [mark=x,corered] table {\pubsubcountfour} ;
				\addplot [mark=x,coreblue] table {\pubsubcountfive} ;
				\addplot [mark=x,coregreen] table {\pubsubcountsix} ;
				\addplot [mark=triangle,corered] table {\pubsubcountseven} ;
				\addplot [mark=triangle,coreblue] table {\pubsubcounteight} ;
				\addplot [mark=triangle,coregreen] table {\pubsubcountnine} ;
				%\addplot [mark=o,coregreen] table {\pubsubcounttenx};

				\legend{1 Publisher,2 Publishers,3 Publishers,4 Publishers,5 Publishers,6 Publishers,7 Publishers,8 Publishers,9 Publishers,10 Publishers}
			\end{axis} 
		\end{tikzpicture}
	\caption{Analysis of the setup time with increasing numbers of publishers and subscribers. In each run another publisher is added that will be subscribed by all subscribers.}
	\label{fig:pubsubcount}
	%\vspace{-7mm}
\end{figure}	

\begin{figure}
	\centering
		\begin{tikzpicture} 

			\begin{axis}[change y base, y SI prefix=milli, y unit=\milli\second, x unit=\mega Bit\per\second,xlabel={\acl{CT}}, ylabel={Setup Time}, xmin=0, xmax=1000, legend style={font=\scriptsize,at={(.05,.95)},anchor=north west}] 

				\addplot [mark=triangle,coregreen] table {\recbarmin} ;
				\addplot [mark=o,coreblue] table {\recbaravg} ;
				\addplot [mark=square,corered] table {\recbarmax} ;

				\legend{Min, Avg/Mean, Max}
			\end{axis} 
		\end{tikzpicture}
	\caption{Analysis of the min max avg setup time in a realistic network with \ac{CT}.}
	\label{fig:recbarctminmax}
	%\vspace{-7mm}
\end{figure}

